ColorSense: A Study on Color Vision in Machine Visual Recognition

Color vision is essential for human visual perception, but its impact on machine perception is still underexplored. There has been an intensified demand for understanding its role in machine perception for safety-critical tasks such as assistive driving and surgery but lacking suitable datasets. To fill this gap, we curate multipurpose datasets ColorSense, by collecting 110,000 non-trivial human annotations of foreground and background color labels from popular visual recognition benchmarks. To investigate the impact of color vision on machine perception, we assign each image a color discrimination level based on its dominant foreground and background colors and use it to study the impact of color vision on machine perception. We validate the use of our datasets by demonstrating that the level of color discrimination has a dominating effect on the performance of mainstream machine perception models. Specifically, we examine the perception ability of machine vision by considering key factors such as model architecture, training objective, model size, training data, and task complexity. Furthermore, to investigate how color and environmental factors affect the robustness of visual recognition in machine perception, we integrate our ColorSense datasets with image corruptions and perform a more comprehensive visual perception evaluation. Our findings suggest that object recognition tasks such as classification and localization are susceptible to color vision bias, especially for high-stakes cases such as vehicle classes, and advanced mitigation techniques such as data augmentation and so on only give marginal improvement. Our analyses highlight the need for new approaches toward the performance evaluation of machine perception models in real-world applications. Lastly, we present various potential applications of ColorSense such as studying spurious correlations.

==> fig_bar_all_datasets.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_barplot_compare_models_on_contrast__cifar10_normal_all_natural_1.pdf}
        \caption{Clean CIFAR10}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_barplot_compare_models_on_contrast__cifar10_normal_all_all_all.pdf}
        \caption{CIFAR10-C}
     \end{subfigure}%\hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_barplot_compare_models_on_contrast__cifar100_normal_all_natural_1.pdf}
        \caption{Clean CIFAR100}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_barplot_compare_models_on_contrast__cifar100_normal_all_all_all.pdf}
        \caption{CIFAR100-C}
     \end{subfigure}%\hfill
    
     \caption{\textbf{Comparing CIFAR10/100 and CIFAR10/100-C by contrast group}. Harder dataset generally shows higher correlation on performance and color contrast.}
     \label{fig:bar_all_datasets}
     \vspace{-5mm}
\end{figure*}

==> fig_cifarb.tex <==
\begin{figure}[t]
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0277.png}
         \caption{black}
     \end{subfigure}% \hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0009.png}
         \caption{blue}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0023.png}
         \caption{green}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0016.png}
         \caption{gray}
     \end{subfigure}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0428.png}
         \caption{red}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0060.png}
         \caption{white}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0047.png}
         \caption{brown}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_b/0292.png}\caption{others}
     \end{subfigure}
     
     \caption{\textbf{Examples of CIFAR10-B (Truck).} CIFAR10-B categorize CIFAR-10 into eight different groups by background colors.}
     \label{fig:examples_cifar10b}
     \vspace{-3mm}
\end{figure}



==> fig_cifarf.tex <==
\begin{figure}[t]
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/black.png}
         \caption{black}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/blue.png}
         \caption{blue}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/green.png}
         \caption{green}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/gray.png}
         \caption{gray}
     \end{subfigure}%\hfill 
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/red.png}
         \caption{red}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/white.png}
         \caption{white}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/brown.png}
         \caption{brown}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.1035\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar_f/others.png}\caption{others}
     \end{subfigure}
     
     \caption{\textbf{Examples of CIFAR10-F (Bird).} We label seven common foreground colors for CIFAR10 and CIFAR100. Difficult examples are categorized as ``others''.}
     \label{fig:examples_cifar10f}
     \vspace{-3mm}
\end{figure}



==> fig_grad_cifar10.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    
     \caption{\textbf{Gradient CIFAR10.} .}
     \label{fig:grad_cifar10}
\end{figure*}

==> fig_grid.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=0.1\linewidth]{figures/gridplot_preResnet101.pdf}
        \caption{\textbf{Accuracy by severity and contrast (preResnet101).}}
        \label{fig:grid_preres101}
        \vspace{-5mm}
\end{figure}
% \vspace{-1mm}

% \begin{wrapfigure}{r}{4.5cm}
%   % \vspace{-6mm}
%   \includegraphics[width=1\linewidth]{figures/gridplot_preResnet101.pdf}
%         \caption{\textbf{Accuracy by severity and contrast (preResnet101).}}
%         \label{fig:grid_preres101}
%         % \vspace{-5mm}
% \end{wrapfigure}

==> fig_label_process.tex <==
\begin{figure}[t]
     \begin{subfigure}[b]{0.12\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/label_process/0185.png}
         \caption{Principle 1}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.12\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/label_process/0010.png}
         \caption{Principle 2}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.12\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/label_process/0336.png}
         \caption{Principle 3}
     \end{subfigure}
     \caption{\textbf{Examples of the three labeling principles for CIFAR-F.} See \S~\ref{sec:labeling} for full labeling details.}
     \label{fig:labeling}
     % \vspace{-3mm}
\end{figure}



==> fig_metrics_imagenet.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         % \caption{Metric 1}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         % \caption{Metric 2}
     \end{subfigure}
     \caption{\textbf{Sensitivity to color contrast and noise severity \ming{need new metrics}.} .}
     \label{fig:metrics}
     \vspace{-5mm}
\end{figure*}

==> fig_objloc_qualitative.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         % \caption{Metric 1}
     \end{subfigure}\hfill
     \begin{subfigure}[t]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         % \caption{Metric 2}
     \end{subfigure}
     \caption{\textbf{Robustness to color vision (\textit{left})and CIFAR10 (\textit{right}).} symbol size is proportional to model size.}
     \label{fig:objloc_car}
     \vspace{-5mm}
\end{figure*}

==> fig_percentChange_cifar10.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_Aug_by_contrast_level_heatmap_PercentChange__cifar10_all_resnet18_natural_1.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_Aug_by_contrast_level_heatmap_PercentChange__cifar10_all_resnet101_natural_1.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_Aug_by_contrast_level_heatmap_PercentChange__cifar10_all_preResnet18_natural_1.pdf}
        % \caption{}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_Aug_by_contrast_level_heatmap_PercentChange__cifar10_all_preResnet101_natural_1.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_Aug_by_contrast_level_heatmap_PercentChange__cifar10_all_preVitTiny224_natural_1.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plot_Aug_by_contrast_level_heatmap_PercentChange__cifar10_all_preVitSmall224_natural_1.pdf}
        % \caption{}
     \end{subfigure}%\hfill
     \caption{\textbf{Percentage (\%) differences in accuracy from DA to normal training by different contrast groups (CIFAR10-CoCo).} (1) On standard Resnets, DA such as Cutmix and Mixup are particularly helpful in lower contrast groups but situation reverses for pre-trained Resnets. (2) on ViTs the help from DAs are not obvious. Our results suggest different DA suits different scenarios.}
     \label{fig:percentChange_cifar10}
     \vspace{-5mm}
\end{figure*}


==> fig_radar_cifar10_cifar100.tex <==
% \begin{figure*}[t]
%       \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_resnet101_all_all.pdf}
%         % \caption{}
%      \end{subfigure}%\hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_preResnet101_all_all.pdf}
%         % \caption{}
%      \end{subfigure}
%     %  \hspace{.9em}
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_preVitSmall224_all_all.pdf}
%         % \caption{}
%      \end{subfigure}%\hfill
   
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_contrast__cifar10_normal_resnet101_all_5.pdf}
%         % \caption{}
%      \end{subfigure}%\hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_contrast__cifar10_normal_preResnet101_all_5.pdf}
%         % \caption{}
%      \end{subfigure}
%     %  \hspace{.9em}
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_contrast__cifar10_normal_preVitSmall224_all_5.pdf}
%         % \caption{}
%      \end{subfigure}%\hfill
%     %  \hspace{.9em}
    
%      \caption{\textbf{Radar plots on CIFAR10-C (severity=5).} We try to understand what causes inconsistencies in Fig.~\ref{fig:reg_cifar100} and Fig.~\ref{fig:reg_cifar10c} and how different contrast groups performs in the presence of different external factors. On Resnets, surprisingly, we find that noises make the distinctions between high to low contrast stand out. For ViTs, the contrast level seems to play a less significant role on different corruption types.}
%      \label{fig:radar_cifar10_cifar100}
%      \vspace{-3mm}
% \end{figure*}

\begin{figure*}[t]
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_contrast__cifar10_normal_resnet18_all_5.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_contrast__cifar10_normal_resnet101_all_5.pdf}
        % \caption{}
     \end{subfigure}%\hfill
     \caption{\textbf{Performance on each corruption by color contrast (severity=5).} We try to understand how different contrast groups performs in the presence of different external factors. On Resnets, surprisingly, we find that color contrast affects noises the most. For ViTs, the contrast level seems to be less significant in general.}
     \label{fig:radar_cifar10_cifar100}
     \vspace{-4mm}
\end{figure*}

==> fig_radar_object_localization.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.48\textwidth}%\label{fig:bar_cifar10}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar10_barplot.png}
        % \caption{}
     \end{subfigure}%\hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_contrast__cifar10_normal_resnet18_all_5.pdf}
        % \caption{}
     \end{subfigure}%\hfill
     \caption{\textbf{CIFAR10 (\textit{left}) and object localization results on \textsc{ColorSense-ImageNet-C} (\textit{right})} \ming{both need re-plot}.}
     \label{fig:radar_obj_loc_imagenet-c}
     \vspace{-5mm}
\end{figure*}

==> fig_reg_cifar10-c.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_resnet18_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_resnet101_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_preResnet18_all_all.jpg}
        % \caption{}
     \end{subfigure}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_preResnet101_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_preVitTiny224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_preVitSmall224_all_all.jpg}
        % \caption{}
     \end{subfigure}%\hfill
     \caption{\textbf{Test accuracy by different levels of color contrast (CIFAR10-CoCo on CIFAR10-C).} (1) We observe similar changes from Fig.~\ref{fig:reg_cifar10} to Fig.~\ref{fig:reg_cifar100} where the harder task, adding corruptions, makes the model more reliant on color contrast signal. (2) on corrupted data we pre-trained Resnets show less reliance on color contrast. (3) ViTs continue to be affected less by color contrast.} 
     \label{fig:reg_cifar10c}
     \vspace{-5mm}
\end{figure*}

==> fig_reg_cifar10.tex <==
\begin{figure}[t]
     \begin{subfigure}[b]{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_densenet201_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
     \begin{subfigure}[b]{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_preDensenet201_natural_1.jpg}
        % \caption{}
     \end{subfigure}
     \begin{subfigure}[b]{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar10_normal_preVitSmall224_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \caption{\textbf{Test accuracy by different levels of color contrast (CIFAR10-CoCo).} Judging from regression analysis, Resnets, even after pre-training, appear to have a higher reliance on color contrast while ViTs have less. This matches common wisdom that CNNs draw more insight from the visual cortex system and ViTs rely less on inductive biases. Surprisingly, pre-training and model size differences on Resnets seem not affecting the reliance trend.}
     \label{fig:reg_cifar10}
     \vspace{-5mm}
\end{figure}


==> fig_reg_cifar100.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar100_normal_resnet18_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar100_normal_resnet101_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar100_normal_preResnet18_natural_1.jpg}
        % \caption{}
     \end{subfigure}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar100_normal_preResnet101_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar100_normal_preVitTiny224_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_regression_by_contrast_per_model__cifar100_normal_preVitSmall224_natural_1.jpg}
        % \caption{}
     \end{subfigure}%\hfill
    
     \caption{\textbf{Test accuracy by different levels of color contrast (CIFAR100-CoCo).} From regression slopes, we observe (1) steeper slopes compared to Fig.~\ref{fig:reg_cifar10} on all tested models. We believe difficult tasks (more classes) makes the model have more reliance on color contrast as a signal, similar to humans. (2) ViTs are significantly less sensitive to color contrast changes (3) We observe significantly smoother slopes on Resnet101 compared to Resnet18, suggesting the benefit of bigger model show up in more complex task for CNNs.}
     \label{fig:reg_cifar100}
     \vspace{-3mm}
\end{figure*}

==> fig_spurious.tex <==
\begin{wrapfigure}{r}{4cm}
    \vspace{-1mm}
    \centering
   \includegraphics[width=0.28\textwidth]{figures/fig52_oneModel_ProtectAttr_imagenet_natrual_resnet50_V1.png}\vspace{-4mm}
     \caption{\textbf{Background and foreground colors as spurious correlations.}\vspace{-3mm}}
     \label{fig:spurious}
     \vspace{-10mm}
\end{wrapfigure}

==> fig_std_gaussian.tex <==
\begin{figure*}[t]
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/fig44_scatterplot_metrics__avg_acc_scaleby_w_std_contrast__avg_acc_scaleby_w_std_severity.png}
         % \caption{Metric 1}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/barplot_cifar10.png}
         % \caption{Metric 2}
     \end{subfigure}
     \caption{\textbf{Robustness to color vision and CIFAR10.} .}
     \label{fig:stds_gauss_cifar10}
     \vspace{-5mm}
\end{figure*}

==> fig_std_imagenet.tex <==
\begin{figure*}[t]
    
     \begin{minipage}[b]{0.3\textwidth}
         % \begin{table}[t] 
            \centering
            
            \captionof{table}{Object localization accuracy. The color vision effect exists in another visual recognition task like object localization, not only in classification.}
            \begin{adjustbox}{width=\linewidth}
            \begin{tabular}{cccc}
            \toprule
            CD Group & IoU-30 & IoU-50 & IoU-70 \\\midrule
            Easy & 75.31 & 73.12 & 50.34 \\
            Medium & 74.48 & 72.77 & 50.01 \\
            Hard & 72.94 & 70.80 & 48.97 \\\bottomrule
            \end{tabular}
            \end{adjustbox}
            \label{tab:obj_loc}
          % \vspace{-5mm}
        % \end{table}
     \end{minipage}\hfill
     \begin{minipage}[b]{0.68\textwidth}
         \begin{subfigure}[t]{0.47\textwidth}
         \centering
         \includegraphics[width=0.85\textwidth]{figures/objLoc_natural_CAR_vs_allcalss_loc30.png}
         % \caption{Metric 2}
        \end{subfigure}\hfill
         \begin{subfigure}[t]{0.51\textwidth}
             \centering
        \includegraphics[width=0.85\textwidth]{figures/fig52_oneModel_ProtectAttr_imagenet_natrual_resnet50_V1.png}
         \end{subfigure}
         \caption{
          \textit{Left:} object localization performance on ImageNet (threshold=IoU-30) --- vehicle classes are more affected by color vision effect. \textit{Right:} background and foreground colors as spurious correlations; green objects/background are favored by \texttt{Resnet50}.
         }
         \label{fig:std_imagenet}
     \end{minipage}
     \vspace{-5mm}
\end{figure*}

==> fig_table_summarize.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=\linewidth]{figures/tab_summary.png}
        \caption{}
        \label{fig:tab_summary}
        \vspace{-5mm}
\end{figure}

==> supp_fig_radar_cifar100_corruption.tex <==
\begin{figure*}[h]
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar100_normal_resnet18_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar100_normal_resnet101_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar100_normal_preResnet18_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar100_normal_preResnet101_all_all.pdf}
        % \caption{}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar100_normal_preVitTiny224_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar100_normal_preVitSmall224_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    
     \caption{\textbf{Performance on each type of corruption in CIFAR100-C by severity.} The behavior on each level of severity and each type of corruption are different. We encourage joint further study on them with our CIFAR100-CoCo.}
     \label{fig:radar_cifar100c}
     \vspace{-3mm}
\end{figure*}

==> supp_fig_radar_cifar10_corruption.tex <==
\begin{figure*}[h]
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_resnet18_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_resnet101_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_preResnet18_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_preResnet101_all_all.pdf}
        % \caption{}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_preVitTiny224_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/polarplot_compare_models_on_corruption__cifar10_normal_preVitSmall224_all_all.pdf}
        % \caption{}
     \end{subfigure}%\hfill
    %  \hspace{.9em}
    
     \caption{\textbf{Performance on each type of corruption in CIFAR10-C by severity.} The behavior on each level of severity and each type of corruption are different. We encourage joint further study on them with our CIFAR10-CoCo.}
     \label{fig:radar_cifar10c}
     \vspace{-3mm}
\end{figure*}

==> supp_tab_cifar10-f.tex <==

\begin{table*}[h]
\centering
  \begin{adjustbox}{max width=\textwidth}
   \begin{tabular}{lcccccccc}
    \toprule
    Classes & Green & Gray & Blue & White & Black & Brown & Red & Others \\
     \midrule
    cat & 0 & 115 & 3 & 85 & 133 & 527 & 0 & 137 \\
    dog & 0 & 19 & 0 & 377 & 114 & 386 & 1 & 103 \\
    truck & 72 & 31 & 135 & 294 & 50 & 102 & 270 & 46 \\
    bird & 43 & 90 & 37 & 102 & 198 & 441 & 37 & 52 \\
    airplane & 108 & 150 & 138 & 298 & 152 & 86 & 45 & 23 \\
    ship & 39 & 61 & 117 & 429 & 98 & 87 & 110 & 59 \\
    frog & 420 & 69 & 8 & 6 & 29 & 396 & 23 & 49 \\
    horse & 6 & 21 & 7 & 288 & 142 & 510 & 3 & 23 \\
    deer & 6 & 46 & 3 & 29 & 75 & 834 & 0 & 7 \\
    automobile & 56 & 129 & 187 & 227 & 116 & 87 & 192 & 6 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{\textbf{CIFAR10-F Statistics.} The number of instances that belongs to each background color from each class.}
  \label{tab:cifar10f_appendix}
\end{table*}


==> supp_tab_cifar100-f.tex <==

\begin{table*}[h]
\centering
  \begin{adjustbox}{max width=\textwidth}
   \begin{tabular}{lcccccccc}
    \toprule
    Classes & Green & Gray & Blue & White & Black & Brown & Red & Others  \\
    
     \midrule
    streetcar & 21 & 2 & 6 & 5 & 3 & 19 & 38 & 6 \\
    apple & 6 & 0 & 0 & 0 & 0 & 9 & 69 & 16 \\
    palm_tree & 95 & 0 & 0 & 0 & 1 & 1 & 0 & 3 \\
    man & 0 & 0 & 0 & 72 & 6 & 5 & 0 & 17 \\
    forest & 53 & 0 & 0 & 0 & 9 & 26 & 1 & 11 \\
    butterfly & 3 & 1 & 6 & 5 & 14 & 58 & 10 & 3 \\
    lamp & 3 & 4 & 8 & 16 & 26 & 32 & 4 & 7 \\
    wardrobe & 0 & 3 & 0 & 13 & 0 & 81 & 2 & 1 \\
    pear & 37 & 1 & 0 & 4 & 0 & 46 & 6 & 6 \\
    raccoon & 0 & 6 & 0 & 5 & 4 & 84 & 1 & 0 \\
    crab & 8 & 2 & 0 & 0 & 9 & 15 & 51 & 15 \\
    tractor & 8 & 1 & 6 & 0 & 0 & 72 & 12 & 1 \\
    aquarium_fish & 0 & 2 & 20 & 3 & 0 & 21 & 28 & 26 \\
    can & 12 & 11 & 10 & 18 & 3 & 11 & 16 & 19 \\
    tank & 55 & 14 & 1 & 0 & 12 & 15 & 0 & 3 \\
    snail & 6 & 6 & 1 & 10 & 0 & 71 & 2 & 4 \\
    bed & 0 & 5 & 11 & 42 & 1 & 16 & 8 & 17 \\
    cup & 10 & 9 & 8 & 14 & 6 & 24 & 3 & 26 \\
    television & 0 & 37 & 3 & 9 & 43 & 7 & 1 & 0 \\
    turtle & 29 & 5 & 13 & 3 & 10 & 33 & 0 & 7 \\
    boy & 0 & 0 & 0 & 72 & 18 & 4 & 0 & 6 \\
    mushroom & 1 & 0 & 0 & 26 & 0 & 65 & 5 & 3 \\
    bee & 0 & 0 & 0 & 1 & 32 & 64 & 0 & 3 \\
    fox & 0 & 0 & 0 & 7 & 0 & 93 & 0 & 0 \\
    willow_tree & 78 & 3 & 2 & 0 & 0 & 12 & 3 & 2 \\
    couch & 8 & 4 & 11 & 22 & 10 & 29 & 7 & 9 \\
    dolphin & 5 & 53 & 19 & 1 & 18 & 4 & 0 & 0 \\
    cattle & 0 & 0 & 0 & 13 & 24 & 55 & 0 & 8 \\
    maple_tree & 58 & 0 & 0 & 1 & 5 & 8 & 24 & 4 \\
    plain & 53 & 2 & 3 & 1 & 2 & 38 & 1 & 0 \\
    bear & 0 & 0 & 0 & 20 & 30 & 49 & 0 & 1 \\
    bridge & 5 & 36 & 1 & 9 & 18 & 20 & 6 & 5 \\
    leopard & 2 & 6 & 0 & 11 & 2 & 77 & 0 & 2 \\
    hamster & 1 & 2 & 0 & 23 & 0 & 74 & 0 & 0 \\
    lawn_mower & 26 & 2 & 0 & 0 & 15 & 8 & 35 & 14 \\
    lobster & 12 & 1 & 8 & 3 & 9 & 20 & 37 & 10 \\
    camel & 0 & 0 & 0 & 17 & 7 & 74 & 0 & 2 \\
    tiger & 0 & 0 & 0 & 3 & 0 & 96 & 0 & 1 \\
    road & 2 & 38 & 0 & 3 & 43 & 14 & 0 & 0 \\
    whale & 0 & 23 & 14 & 7 & 54 & 2 & 0 & 0 \\
    motorcycle & 5 & 0 & 21 & 6 & 19 & 13 & 25 & 11 \\
    crocodile & 50 & 1 & 4 & 4 & 10 & 29 & 1 & 1 \\
    dinosaur & 37 & 2 & 7 & 1 & 2 & 40 & 4 & 7 \\
    chair & 6 & 5 & 11 & 8 & 8 & 49 & 10 & 3 \\
    bus & 7 & 6 & 11 & 30 & 1 & 24 & 13 & 8 \\
    plate & 8 & 1 & 13 & 34 & 1 & 11 & 1 & 31 \\
    otter & 6 & 3 & 0 & 11 & 6 & 74 & 0 & 0 \\
    rose & 0 & 0 & 1 & 7 & 0 & 10 & 80 & 2 \\
    seal & 4 & 4 & 5 & 19 & 8 & 56 & 0 & 4 \\
    telephone & 1 & 7 & 11 & 23 & 50 & 7 & 1 & 0 \\
    mouse & 3 & 16 & 0 & 11 & 5 & 62 & 2 & 1 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{\textbf{CIFAR100-F Statistics (part 1).} The number of instances that belongs to each foreground color from each class.}
  \label{tab:cifar100b_appendix}
\end{table*}


\begin{table*}[h]
\centering
  \begin{adjustbox}{max width=\textwidth}
   \begin{tabular}{lcccccccc}
    \toprule
    Classes & Green & Gray & Blue & White & Black & Brown & Red & Others  \\
     \midrule
        
    tulip & 0 & 0 & 5 & 12 & 0 & 22 & 61 & 0 \\
    porcupine & 0 & 4 & 0 & 1 & 8 & 85 & 0 & 2 \\
    beaver & 0 & 7 & 0 & 0 & 10 & 82 & 0 & 1 \\
    wolf & 0 & 31 & 0 & 17 & 4 & 48 & 0 & 0 \\
    lizard & 37 & 7 & 3 & 1 & 0 & 32 & 2 & 18 \\
    flatfish & 10 & 5 & 2 & 22 & 5 & 52 & 1 & 3 \\
    beetle & 30 & 2 & 7 & 0 & 18 & 13 & 22 & 8 \\
    chimpanzee & 0 & 7 & 0 & 1 & 59 & 33 & 0 & 0 \\
    poppy & 0 & 0 & 3 & 3 & 0 & 35 & 56 & 3 \\
    bowl & 10 & 0 & 8 & 17 & 4 & 19 & 7 & 35 \\
    table & 6 & 4 & 3 & 25 & 0 & 58 & 2 & 2 \\
    shrew & 0 & 3 & 0 & 2 & 18 & 77 & 0 & 0 \\
    skyscraper & 6 & 33 & 44 & 0 & 9 & 8 & 0 & 0 \\
    kangaroo & 0 & 3 & 0 & 9 & 7 & 81 & 0 & 0 \\
    cloud & 0 & 5 & 7 & 74 & 6 & 1 & 5 & 2 \\
    girl & 0 & 0 & 0 & 79 & 11 & 10 & 0 & 0 \\
    worm & 18 & 6 & 16 & 4 & 10 & 32 & 11 & 3 \\
    train & 13 & 7 & 13 & 0 & 10 & 23 & 15 & 19 \\
    house & 6 & 4 & 6 & 27 & 0 & 35 & 3 & 19 \\
    caterpillar & 45 & 0 & 1 & 6 & 8 & 10 & 8 & 22 \\
    spider & 6 & 0 & 3 & 5 & 19 & 34 & 0 & 33 \\
    rabbit & 0 & 4 & 0 & 33 & 10 & 52 & 0 & 1 \\
    cockroach & 2 & 0 & 2 & 0 & 32 & 58 & 3 & 3 \\
    rocket & 11 & 10 & 2 & 43 & 20 & 7 & 1 & 6 \\
    castle & 0 & 22 & 1 & 32 & 0 & 42 & 1 & 2 \\
    bicycle & 10 & 10 & 11 & 5 & 27 & 4 & 13 & 20 \\
    baby & 0 & 0 & 0 & 63 & 8 & 7 & 16 & 6 \\
    mountain & 15 & 10 & 7 & 43 & 2 & 19 & 1 & 3 \\
    sweet_pepper & 29 & 0 & 0 & 0 & 0 & 27 & 25 & 19 \\
    orchid & 5 & 0 & 1 & 31 & 0 & 7 & 53 & 3 \\
    sea & 2 & 12 & 64 & 5 & 7 & 2 & 0 & 8 \\
    skunk & 0 & 0 & 0 & 1 & 79 & 19 & 0 & 1 \\
    oak_tree & 96 & 0 & 0 & 0 & 2 & 2 & 0 & 0 \\
    squirrel & 1 & 12 & 0 & 2 & 7 & 78 & 0 & 0 \\
    ray & 10 & 23 & 21 & 9 & 14 & 12 & 1 & 10 \\
    bottle & 19 & 1 & 1 & 1 & 13 & 32 & 5 & 28 \\
    pickup_truck & 7 & 6 & 15 & 16 & 12 & 14 & 28 & 2 \\
    keyboard & 5 & 13 & 9 & 46 & 17 & 4 & 0 & 6 \\
    lion & 0 & 3 & 0 & 2 & 1 & 94 & 0 & 0 \\
    clock & 1 & 2 & 15 & 15 & 15 & 41 & 8 & 3 \\
    trout & 30 & 10 & 4 & 10 & 2 & 28 & 4 & 12 \\
    orange & 0 & 0 & 0 & 0 & 0 & 98 & 2 & 0 \\
    woman & 0 & 0 & 0 & 36 & 49 & 14 & 0 & 1 \\
    shark & 8 & 24 & 29 & 20 & 8 & 7 & 1 & 3 \\
    sunflower & 1 & 0 & 0 & 1 & 0 & 96 & 2 & 0 \\
    pine_tree & 80 & 2 & 0 & 3 & 13 & 1 & 0 & 1 \\
    snake & 21 & 4 & 4 & 0 & 18 & 23 & 11 & 19 \\
    elephant & 0 & 73 & 0 & 1 & 25 & 1 & 0 & 0 \\
    possum & 0 & 20 & 3 & 10 & 6 & 58 & 0 & 3 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{\textbf{CIFAR100-F Statistics (part 2).} The number of instances that belongs to each foreground color from each class.}
  \label{tab:cifar100b_appendix}
\end{table*}




==> tab_gap_imagenet.tex <==
\begin{table}[t]
    \centering
    \vspace{-2mm}
    \caption{Average absolute gap by architecture type and dataset.\vspace{-0mm}}
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{cccccccccc}
    \toprule
    Absolute Gap & Conv. & Mob.& Mob(adv) & Res. & Res(adv) & Resx. & Resx(adv) & SwinV2 & ViT \\\midrule
    \textsc{ColorSense} & 2.17 & 2.86 & 2.62 & 3.12 & 2.21 & 2.97 & 2.56 & 2.18 & 2.48 \\
    Land vehicle-only & 3.40 & 4.35 & 4.87 & 6.59 & 4.27 & 4.63 & 5.87 & 4.31 & 6.93  \\\hline
    \textsc{ColorSense-C} & 4.59 & 3.37 & n/a & 4.40 & n/a & 4.46 & n/a & 4.40 & 4.64 \\\bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:AG}
    \vspace{-5mm}
\end{table}
  
% \begin{table}[ht]
%     % \vspace{-2mm}
%   \begin{subtable}[t]{\linewidth} % Adjust the width as needed
%     \centering
%     \vspace{-4mm}
%     \begin{adjustbox}{width=\textwidth}
%     \begin{tabular}{cccccccccc}
%     \toprule
%     Absolute Gap & Conv. & Mob.& Mob(adv) & Res. & Res(adv) & Resx. & Resx(adv) & SwinV2 & ViT \\\midrule
%     \textsc{ColorSense} & 2.17 & 2.86 & 2.62 & 3.12 & 2.21 & 2.97 & 2.56 & 2.18 & 2.48 \\
%     Land vehicle-only & 3.40 & 4.35 & 4.87 & 6.59 & 4.27 & 4.63 & 5.87 & 4.31 & 6.93  \\\hline
%     \textsc{ColorSense-C} & 4.59 & 3.37 & n/a & 4.40 & n/a & 4.46 & n/a & 4.40 & 4.64 \\\bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Table 2a: Average absolute gap by architecture type and dataset.\vspace{-0mm}}
%     \label{tab:table1}
%   \end{subtable}%
  
%   \begin{subtable}[t]{0.5\linewidth} % Adjust the width as needed
%     \centering
%     % \vspace{-4mm}
%     \begin{adjustbox}{width=\textwidth}
%     \begin{tabular}{cccc}
%     \toprule
%     CD Group & IoU-30 & IoU-50 & IoU-70 \\\midrule
%     Easy & 75.31 & 73.12 & 50.34 \\
%     Medium & 74.48 & 72.77 & 50.01 \\
%     Hard & 72.94 & 70.80 & 48.97 \\\bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Table 2b: Obj. localization acc.\vspace{-0mm}}
%     \label{tab:table2}
%   \end{subtable}
%   \vspace{-4mm}
% \end{table}






==> tab_modelSize.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cc}\toprule
        Model &  \#parameters \\\midrule
        Resnet18 & 11.4M\\
        Resnet101 & 42.8M\\\midrule
        Densenet121 & 8M\\
        Densenet201 & 20M\\\midrule
        ViT Tiny & 5M\\
        ViT Small & 22M\\\bottomrule
    \end{tabular}
    \caption{Model size of tested architectures.}
    \label{tab:model_size}
\end{table}


% \begin{wraptable}{r}{4cm}
% \vspace{-3mm}
% \begin{tabular}{cc}\toprule
%         Model &  \#parameters \\\midrule
%         Resnet18 & 11.4M\\
%         Resnet101 & 42.8M\\\midrule
%         Densenet121 & 8M\\
%         Densenet201 & 20M\\\midrule
%         ViT Tiny & 5M\\
%         ViT Small & 22M\\\bottomrule
%     \end{tabular}
%     \caption{Model size of tested architectures.}
%     \label{tab:model_size}
% \end{wraptable}

==> tab_object_loc.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.55\textwidth}
    \includegraphics[width=\textwidth]{figures/barplot_cifar10.png}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.45\textwidth}
   \centering
    \begin{tabular}{cccc}
    \toprule
    CD Group & IoU-30 & IoU-50 & IoU-70 \\\midrule
    Easy & 75.31 & 73.12 & 50.34 \\
    Medium & 74.48 & 72.77 & 50.01 \\
    Hard & 72.94 & 70.80 & 48.97 \\\bottomrule
    \end{tabular}
  \end{subfigure}
  \caption{\textbf{CIFAR10 (\textit{left}) and Object localization accuracy by threshold (\textit{right}).} \ming{don't know how to make the plot right} \ming{debating what models to show for CIFAR10} Color vision still affect recognition on smaller CIFAR10 dataset and object localization performance.}
  \label{tab:object-localization}
\end{figure}

==> tab_std_imagenet.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{ccccc}
    \toprule
        wstd & Resnt & ViTx & Swin  \\\midrule
        Hard & 7 & & 2820 \\
        Medium & 6 & & 212\\
        Easy & 9 & & 2615 \\\bottomrule
    \end{tabular}
    \caption{Slope of to color vision groups measured by weighted standard deviation. }
    \label{tab:slope-imagenet}
    % \vspace{-5mm}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccccc}
%     \toprule
%         wstd & Resnt & ViTx & Swin  \\\midrule
%         Hard & 7 & & 2820 \\
%         Medium & 6 & & 212\\
%         Easy & 9 & & 2615 \\\bottomrule
%     \end{tabular}
%     \caption{Sensitivity to color vision groups measured by weighted standard deviation. }
%     \label{tab:sensitivity-imagenet}
%     % \vspace{-5mm}
% \end{table}


